Adaptive Recovery of Dictionary-sparse Signals using Binary Measurements

One-bit compressive sensing (CS) is an advanced version of sparse recovery in which the sparse signal of interest can be recovered from extremely quantized measurements. Namely, only the sign of each measurement is available to us. In many applications, the ground-truth signal is not sparse itself, but can be represented in a redundant dictionary. A strong line of research has addressed conventional CS in this signal model including its extension to one-bit measurements. However, one-bit CS suffers from the extremely large number of required measurements to achieve a predefined reconstruction error level. A common alternative to resolve this issue is to exploit adaptive schemes. Adaptive sampling acts on the acquired samples to trace the signal in an efficient way. In this work, we utilize an adaptive sampling strategy to recover dictionary-sparse signals from binary measurements. For this task, a multi-dimensional threshold is proposed to incorporate the previous signal estimates into the current sampling procedure. This strategy substantially reduces the required number of measurements for exact recovery. Our proof approach is based on the recent tools in high dimensional geometry in particular random hyperplane tessellation and Gaussian width. We show through rigorous and numerical analysis that the proposed algorithm considerably outperforms state of the art approaches. Further, our algorithm reaches an exponential error decay in terms of the number of quantized measurements.

==> Figures/SimFig1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=20000,
xlabel style={font=\color{white!15!black}},
xlabel={Number of measurments},
ymin=-70,
ymax=0,
ylabel style={font=\color{white!15!black}},
ylabel={Nomalized reconstruction error (dB)},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black!50!green, dashdotted, line width=1.5pt, mark=asterisk, mark options={solid, black!50!green}]
  table[row sep=crcr]{%
100	-0.7911609623564\\
600	-3.85221419151128\\
1100	-6.15311901503681\\
1600	-6.83357183188903\\
2100	-8.46790666763119\\
2600	-9.13829297336606\\
3100	-9.91027380727408\\
3600	-10.4641226865645\\
4100	-11.2116482328564\\
4600	-11.536532935649\\
5100	-11.3979931769735\\
5600	-12.0949605696561\\
6100	-12.4860448954269\\
6600	-12.4249079032032\\
7100	-13.3819926144739\\
7600	-13.4470535132629\\
8100	-13.5631460491734\\
8600	-14.4272250151355\\
9100	-14.3352872723795\\
9600	-14.4454607268224\\
10100	-14.9293194227767\\
10600	-15.0622070994623\\
11100	-15.0108674030056\\
11600	-15.3468897130173\\
12100	-15.4969992631846\\
12600	-15.8485747333295\\
13100	-15.7076387397019\\
13600	-16.008309143618\\
14100	-16.0927382263638\\
14600	-16.5244682999027\\
15100	-16.4245263176834\\
15600	-15.9419721015168\\
16100	-16.7156968958872\\
16600	-16.6679689502404\\
17100	-16.8181489865382\\
17600	-16.9323746346529\\
18100	-17.6392413737559\\
18600	-17.6590084119863\\
19100	-17.3885220928064\\
19600	-17.4558286072471\\
};
\addlegendentry{LP}

\addplot [color=red, dashed, line width=1.5pt, mark=diamond, mark options={solid, red}]
  table[row sep=crcr]{%
100	-0.580502013290548\\
600	-3.17378648520666\\
1100	-5.06598456805811\\
1600	-5.98504510721052\\
2100	-7.31978380964953\\
2600	-7.99074777449843\\
3100	-8.48575432020161\\
3600	-9.30289332820336\\
4100	-9.86167435687212\\
4600	-10.3928830369121\\
5100	-10.3729746602429\\
5600	-11.065252114284\\
6100	-10.9024308166853\\
6600	-11.4927812206428\\
7100	-11.9403558416938\\
7600	-11.9224113767993\\
8100	-12.3013128422292\\
8600	-13.2798195666559\\
9100	-13.2100259356084\\
9600	-13.1292393572542\\
10100	-13.7502214023833\\
10600	-13.7033109138065\\
11100	-13.7558627414811\\
11600	-13.8964193313831\\
12100	-14.2224246173695\\
12600	-14.3521820645841\\
13100	-14.2876405820904\\
13600	-14.7384025390748\\
14100	-14.7624419883146\\
14600	-15.1468695773253\\
15100	-15.1590947554043\\
15600	-14.9764127736858\\
16100	-15.0311896640051\\
16600	-15.3213662872021\\
17100	-15.552971436663\\
17600	-15.6045088927994\\
18100	-16.4989023988085\\
18600	-16.2392472949893\\
19100	-16.1261732810351\\
19600	-16.0870011591663\\
};
\addlegendentry{CP}

\addplot [color=blue, line width=1.5pt, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
100	-0.147947365682645\\
600	-1.065549367255\\
1100	-2.08235476397102\\
1600	-3.68209151459224\\
2100	-4.49500966386939\\
2600	-6.16703391743265\\
3100	-8.18292489456517\\
3600	-9.80078786731078\\
4100	-10.9228921687073\\
4600	-13.7266571479186\\
5100	-17.1234810879131\\
5600	-18.7578997342616\\
6100	-21.9099853688315\\
6600	-28.7408387784407\\
7100	-31.7199755871746\\
7600	-38.7556336187637\\
8100	-42.6130082153605\\
8600	-48.0443229573325\\
9100	-60.001257140286\\
9600	-61.1319213562897\\
10100	-63.6285040688903\\
10600	-63.9423825958842\\
11100	-64.1517242085625\\
11600	-64.4215082990764\\
12100	-65.021075816031\\
12600	-64.9828316564846\\
13100	-65.0823197305787\\
13600	-65.398202244035\\
14100	-65.4115119258461\\
14600	-65.849514943976\\
15100	-66.0055813558248\\
15600	-65.8713649289899\\
16100	-66.2553835524622\\
16600	-66.5725245878359\\
17100	-66.744212621923\\
17600	-66.6775068368816\\
18100	-67.5471840089208\\
18600	-67.5514765822278\\
19100	-67.2010001397537\\
19600	-67.2164143925253\\
};
\addlegendentry{Our algorithm}

\end{axis}
\end{tikzpicture}%

==> Figures/SimFig2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=20000,
xlabel style={font=\color{white!15!black}},
xlabel={Number of measurments},
ymin=-70,
ymax=0,
ylabel style={font=\color{white!15!black}},
ylabel={Nomalized reconstruction error (dB)},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black!50!green, dashdotted, line width=1.5pt, mark=o, mark options={solid, black!50!green}]
  table[row sep=crcr]{%
100	-5.31017788249262e-05\\
1100	-2.50187425425394\\
2100	-6.06394357390255\\
3100	-10.4943989782368\\
4100	-16.7857731264863\\
5100	-23.1799447874167\\
6100	-35.5517884537765\\
7100	-47.7078724197745\\
8100	-54.1197805447874\\
9100	-56.2185600131729\\
10100	-56.6916034094664\\
11100	-57.3442865324729\\
12100	-57.856568787158\\
13100	-58.2995972482567\\
14100	-58.6641274825341\\
15100	-59.1439365288212\\
16100	-59.5011096119874\\
17100	-59.8710206304102\\
18100	-60.1514706230771\\
19100	-60.4761583040337\\
};
\addlegendentry{s=10}

\addplot [color=red, dashed, line width=1.5pt, mark=asterisk, mark options={solid, red}]
  table[row sep=crcr]{%
100	-6.27486524956903e-05\\
1100	-2.55348271202791\\
2100	-5.96390500941153\\
3100	-10.7914794429888\\
4100	-16.4878071671755\\
5100	-24.0419514072612\\
6100	-34.907770814818\\
7100	-48.1810535532371\\
8100	-52.7766596021068\\
9100	-54.267104737645\\
10100	-55.3432224304723\\
11100	-55.9452609100348\\
12100	-56.6459392450339\\
13100	-56.8716343071169\\
14100	-57.2993866042238\\
15100	-57.6900575715803\\
16100	-58.0443331134806\\
17100	-58.3129589311012\\
18100	-58.73553717925\\
19100	-58.7626448341796\\
};
\addlegendentry{s=20}

\addplot [color=green, dotted, line width=1.5pt, mark=triangle, mark options={solid, green}]
  table[row sep=crcr]{%
100	-0.000101266167751299\\
1100	-2.70662321818244\\
2100	-6.28218547060409\\
3100	-10.3860608069949\\
4100	-16.0373933212551\\
5100	-25.2338786217104\\
6100	-35.2614730283202\\
7100	-47.2212884842324\\
8100	-51.7049220721939\\
9100	-53.4190290398514\\
10100	-54.3207211854444\\
11100	-55.1373998201428\\
12100	-55.4103448418634\\
13100	-56.0027308574085\\
14100	-56.5227948414818\\
15100	-56.5806677982956\\
16100	-57.1449981525402\\
17100	-57.5619486112062\\
18100	-57.8549771275769\\
19100	-57.7994166470983\\
};
\addlegendentry{s=30}

\addplot [color=blue, line width=1.5pt, mark=diamond, mark options={solid, blue}]
  table[row sep=crcr]{%
100	-0.000111917480387534\\
1100	-2.36813124762606\\
2100	-6.02637391524806\\
3100	-11.0180528397877\\
4100	-16.6965282670793\\
5100	-23.6463212965025\\
6100	-34.7387276277242\\
7100	-46.2777938047612\\
8100	-51.0036060016498\\
9100	-52.5088500316849\\
10100	-53.6579986055174\\
11100	-54.6187709806697\\
12100	-54.8108141706404\\
13100	-55.2925653681873\\
14100	-55.6516668235334\\
15100	-55.9536349606597\\
16100	-56.3009868506228\\
17100	-56.7324328131441\\
18100	-56.7861318965677\\
19100	-57.1496459709036\\
};
\addlegendentry{s=40}

\addplot [color=mycolor1, dashdotted, line width=1.5pt, mark=square, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
100	-9.8393669956838e-05\\
1100	-2.50066311300693\\
2100	-6.16875406233638\\
3100	-10.630076180413\\
4100	-16.4282519752118\\
5100	-23.6933365659303\\
6100	-33.8365461880566\\
7100	-44.9668577295688\\
8100	-50.7174791793789\\
9100	-52.7136914523257\\
10100	-53.0419330151674\\
11100	-53.7074911435796\\
12100	-54.3487868104918\\
13100	-54.706258501937\\
14100	-55.0871022486169\\
15100	-55.8307717346228\\
16100	-55.8171391259611\\
17100	-56.0782218107797\\
18100	-56.474450705027\\
19100	-56.7695070902359\\
};
\addlegendentry{s=50}

\end{axis}
\end{tikzpicture}%

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

